Design and Operation Principles of a Wave-Controlled Reconfigurable Intelligent Surface

A Reflective Intelligent Surface (RIS) consists of many small reflective elements whose reflection properties can be adjusted to change the wireless propagation environment. Envisioned implementations require that each RIS element be connected to a controller, and as the number of RIS elements on a surface may be on the order of hundreds or more, the number of required electrical connectors creates a difficult wiring problem, especially at high frequencies where the physical space between the elements is limited. A potential solution to this problem was previously proposed by the authors in which "biasing transmission lines" carrying standing waves are sampled at each RIS location to produce the desired bias voltage for each RIS element. This solution has the potential to substantially reduce the complexity of the RIS control. This paper presents models for the RIS elements that account for mutual coupling and realistic varactor characteristics, as well as circuit models for sampling the transmission line to generate the RIS control signals. For the latter case, the paper investigates two techniques for conversion of the transmission line standing wave voltage to the varactor bias voltage, namely an envelope detector and a sample-and-hold circuit. The paper also develops a modal decomposition approach for generating standing waves that are able to generate beams and nulls in the resulting RIS radiation pattern that maximize either the Signal-to-Noise Ratio (SNR) or the Signal-to-Leakage-plus-Noise Ratio (SLNR). Extensive simulation results are provided for the two techniques, together with a discussion of computational complexity.

==> arraymac.tex <==
% general purpose macros fo use with LaTeX (or TeX)
\makeatletter
\newfont{\sqi}{cmssqi8}
\newcommand{\IR}{\mbox{$I\!\!R$}}
\newcommand{\IC}{\mbox{$C\!\!\!\!\raisebox{.75pt}{\mbox{\sqi I}}\;\,$}}
\def\defnas{\stackrel{\rm def}{=}}
\newcommand\vdashl{\vdshl{1}{1}}
\newcommand\bvdashl{\vdshl{1.6}{2}}
\newlength{\tmpln}
\newlength{\dshln}
\newcommand{\vdshl}[2]{{\setbox1=\hbox{$[$}\setlength{\tmpln}{#1\ht1}
\advance\tmpln by #1\dp1
\setlength{\dshln}{.111\tmpln}
\newcommand\vs{\vskip .111\tmpln plus 1pt minus 1pt}
\newcommand\vd{\hrule width .4pt height \dshln depth 0pt}
\setbox2=\hbox{
 \vbox to\tmpln{\lineskip 0pt \lineskiplimit-1000pt \baselineskip 0pt
 \vd\vs\vd\vs\vd\vs\vd\vs\vd\vfil}$\;$}
 \lower#2\dp1\copy2
}}
\newcommand\adots{\mathinner{\mskip0mu\raise0pt\vbox{\kern7pt\hbox{.}}\mskip3mu
    \raise4pt\hbox{.}\mskip3mu\raise8pt\hbox{.}\mskip0mu}}
\def\nonumfootnotetext{\xdef \@thefnmark{}\@footnotetext}
\def\ie{{\it i.e.,\ }}
\def\cf{{\it cf.\ }}
\def\etc{{\it etc.}}
\def\etal{{\it et al.}}
\def\eg{{\it e.g.,\ }}
\def\apriori{{\it a~priori}}
\def\qed{%
   {%
      \unskip
      \nobreak \hfil
      \penalty 50               % TeX should break here if necessary
      \hskip 3em                % mimium amount of distance
      \null \nobreak \hfil
      \qedbox
      \parfillskip=\z@skip
      \finalhyphendemerits=\z@  % no line break at last line of paragraph
      \endgraf                  % don't know what \par is in this moment...
   }}
\def\qedbox{\rule[-1pt]{8pt}{8pt}}\def\QED{\qed}
%\def\beq{\@ifnextchar [{\@tempswatrue\@beq}{\@tempswafalse\@beq[]}}
%\def\@beq[#1]{\begin{equation}\edef\@tmparg{#1}\ifx\@tmparg\@empty \else
%        \label{#1}\fi}
\def\beq[#1]{\begin{equation} \label{#1}}
\newcommand{\eeq}{\end{equation}}
%\def\eeq{\end{equation}}
% \jot 2ex
\newcount\@eqcnt
\newcount\@eqpen
\newif\if@eqnsw\@eqnswtrue
\def\eqnarray{\stepcounter{equation}\let\@currentlabel=\theequation
\global\@eqnswtrue
\global\@eqcnt\z@\tabskip\@centering\let\\=\@eqncr
$$\halign to \displaywidth\bgroup\@eqnsel\hskip\@centering
  $\displaystyle\tabskip\z@{##}$&\global\@eqcnt\@ne
  \hskip .6\arraycolsep \hfil${##}$\hfil
  &\global\@eqcnt\tw@ \hskip .6\arraycolsep $\displaystyle\tabskip\z@{##}$\hfil
   \tabskip\@centering&\llap{##}\tabskip\z@\cr}
\def\str{\rule[-.6em]{0pt}{2.4em}}
\def\proof{\noindent {\bf Proof:\ }}
\let\pbox=\qed
\def\dag{{\cal y}}
\def\phstar{{\phantom{*}}}
\def\dmax{d_{\rm max}}
\def\vcv{\vdashl\cdots\vdashl}
\def\alphabf{{\boldsymbol \alpha}}
\def\betabf{{\boldsymbol \beta}}
\def\gammabf{{\boldsymbol \gamma}}
\def\deltabf{{\boldsymbol \delta}}
\def\epsilonbf{{\boldsymbol \epsilon}}
\def\epsbf{{\boldsymbol \epsilon}}
\def\zetabf{{\boldsymbol \zeta}}
\def\etabf{{\boldsymbol \eta}}
\def\thetabf{{\boldsymbol \theta}}
\def\iotabf{{\boldsymbol \iota}}
\def\kappabf{{\boldsymbol \kappa}}
\def\lambdabf{{\boldsymbol \lambda}}
\def\mubf{{\boldsymbol \mu}}
\def\nubf{{\boldsymbol \nu}}
\def\xibf{{\boldsymbol \xi}}
\def\pibf{{\boldsymbol \pi}}
\def\varphibf{{\boldsymbol \varphi}}
\def\rhobf{{\boldsymbol \rho}}
\def\sigmabf{{\boldsymbol \sigma}}
\def\taubf{{\boldsymbol \tau}}
\def\taubfh{\hat{\taubf}}
\def\upsilonbf{{\boldsymbol \upsilon}}
\def\phibf{{\boldsymbol \phi}}
\def\chibf{{\boldsymbol \chi}}
\def\psibf{{\boldsymbol \psi}}
\def\omegabf{{\boldsymbol \omega}}
\def\Gammabf{{\boldsymbol \Gamma}}
\def\Thetabf{{\boldsymbol \Theta}}
\def\Lambdabf{{\boldsymbol \Lambda}}
\def\Xibf{{\boldsymbol \Xi}}
\def\Pibf{{\boldsymbol \Pi}}
\def\Sigmabf{{\boldsymbol \Sigma}}
\def\Upsilonbf{{\boldsymbol \Upsilon}}
\def\Phibf{{\boldsymbol \Phi}}
\def\Psibf{{\boldsymbol \Psi}}
\def\Psibar{{\bar{\Psibf}}}
\def\Ebar{{\bar{\Ebf}}}
\def\Omegabf{{\boldsymbol \Omega}}
\def\Deltabf{{\boldsymbol \Delta}}
\def\abf{{\bf a}}
\def\bbf{{\bf b}}
\def\cbf{{\bf c}}
\def\dbf{{\bf d}}
\def\ebf{{\bf e}}
\def\fbf{{\bf f}}
\def\gbf{{\bf g}}
\def\hbf{{\bf h}}
\def\ibf{{\bf i}}
\def\iibf{{\bf ii}}
\def\iiibf{{\bf iii}}
\def\jbf{{\bf j}}
\def\kbf{{\bf k}}
\def\lbf{{\bf l}}
\def\ellbf{{\bf \ell}}
\def\mbf{{\bf m}}
\def\nbf{{\bf n}}
\def\obf{{\bf o}}
\def\peebf{{\bf p}}
\def\qbf{{\bf q}}
\def\rbf{{\bf r}}
\def\sbf{{\bf s}}
\def\tbf{{\bf t}}
\def\ubf{{\bf u}}
\def\vbf{{\bf v}}
\def\wbf{{\bf w}}
\def\xbf{{\bf x}}
\def\ybf{{\bf y}}
\def\zbf{{\bf z}}
\def\rbf{{\bf r}}
\def\xbf{{\bf x}}
\def\ybf{{\bf y}}
\def\Abf{{\bf A}}
\def\Bbf{{\bf B}}
\def\Cbf{{\bf C}}
\def\Dbf{{\bf D}}
\def\Ebf{{\bf E}}
\def\Fbf{{\bf F}}
\def\Gbf{{\bf G}}
\def\Hbf{{\bf H}}
\def\Ibf{{\bf I}}
\def\Jbf{{\bf J}}
\def\Kbf{{\bf K}}
\def\Lbf{{\bf L}}
\def\Mbf{{\bf M}}
\def\Nbf{{\bf N}}
\def\Obf{{\bf O}}
\def\Pbf{{\bf P}}
\def\Qbf{{\bf Q}}
\def\Rbf{{\bf R}}
\def\Sbf{{\bf S}}
\def\Tbf{{\bf T}}
\def\Ubf{{\bf U}}
\def\Vbf{{\bf V}}
\def\Wbf{{\bf W}}
\def\Xbf{{\bf X}}
\def\Ybf{{\bf Y}}
\def\Zbf{{\bf Z}}
\def\sf{\mathsf}
\def\asf{{\sf a}}
\def\bsf{{\sf b}}
\def\csf{{\sf c}}
\def\dsf{{\sf d}}
\def\esf{{\sf e}}
\def\fsf{{\sf f}}
\def\gsf{{\sf g}}
\def\hsf{{\sf h}}
\def\isf{{\sf i}}
\def\iisf{{\sf ii}}
\def\iiisf{{\sf iii}}
\def\jsf{{\sf j}}
\def\ksf{{\sf k}}
\def\lsf{{\sf l}}
\def\ellsf{{\sf \ell}}
\def\msf{{\sf m}}
\def\nsf{{\sf n}}
\def\osf{{\sf o}}
\def\psf{{\sf p}}
\def\qsf{{\sf q}}
\def\rsf{{\sf r}}
\def\ssf{{\sf s}}
\def\tsf{{\sf t}}
\def\usf{{\sf u}}
\def\vsf{{\sf v}}
\def\wsf{{\sf w}}
\def\xsf{{\sf x}}
\def\ysf{{\sf y}}
\def\zsf{{\sf z}}
\def\rsf{{\sf r}}
\def\xsf{{\sf x}}
\def\ysf{{\sf y}}
\def\Asf{{\sf A}}
\def\Bsf{{\sf B}}
\def\Csf{{\sf C}}
\def\Dsf{{\sf D}}
\def\Esf{{\sf E}}
\def\Fsf{{\sf F}}
\def\Gsf{{\sf G}}
\def\Hsf{{\sf H}}
\def\Isf{{\sf I}}
\def\Jsf{{\sf J}}
\def\Ksf{{\sf K}}
\def\Lsf{{\sf L}}
\def\Msf{{\sf M}}
\def\Nsf{{\sf N}}
\def\Osf{{\sf O}}
\def\Psf{{\sf P}}
\def\Qsf{{\sf Q}}
\def\Rsf{{\sf R}}
\def\Ssf{{\sf S}}
\def\Tsf{{\sf T}}
\def\Usf{{\sf U}}
\def\Vsf{{\sf V}}
\def\Wsf{{\sf W}}
\def\Xsf{{\sf X}}
\def\Ysf{{\sf Y}}
\def\Zsf{{\sf Z}}
\def\CRB{{\bf CRB}}
\def\FIM{{\bf FIM}}
\def\Ac{{\cal A}}
\def\Bc{{\cal B}}
\def\Cc{{\cal C}}
\def\Dc{{\cal D}}
\def\Ec{{\cal E}}
\def\Fc{{\cal F}}
\def\Gc{{\cal G}}
\def\Hc{{\cal H}}
\def\Ic{{\cal I}}
\def\Jc{{\cal J}}
\def\Kc{{\cal K}}
\def\Lc{{\cal L}}
\def\Mc{{\cal M}}
\def\Nc{{\cal N}}
\def\Oc{{\cal O}}
\def\Pc{{\cal P}}
\def\Qc{{\cal Q}}
\def\Rc{{\cal R}}
\def\Sc{{\cal S}}
\def\Tc{{\cal T}}
\def\Uc{{\cal U}}
\def\Vc{{\cal V}}
\def\Wc{{\cal W}}
\def\Xc{{\cal X}}
\def\Yc{{\cal Y}}
\def\Zc{{\cal Z}}
\def\xbfhat{\hat{\xbf}}
\def\lambdahat{\hat{\lambda}}
\def\lh{\hat{\lambda}}
\def\dh{\hat{d}}
\def\sh{\hat{s}}
\def\sdhh{\hat{\hat{s}}_d}
\def\wh{\hat{\wbf}}
\def\Phibar{\bar{\Phibf}}
\def\lambdatilde{\tilde{\lambda}}
\def\lambdabfhat{\hat{\lambdabf}}
\def\lambdatbf{{\tilde {\lambdabf}}}
\def\At{{\tilde{\Abf}}}
\def\Bt{{\tilde{\Bbf}}}
\def\Ath{{\hat{\tilde{\Abf}}}}
\def\Gt{{\tilde{\Gbf}}}
\def\Tt{{\tilde{\T}}}
\def\Ah{{\hat{\Abf}}}
\def\Gh{{\hat{\Gbf}}}
\def\Qh{{\hat{\Qbf}}}
\def\Th{{\hat{\T}}}
\def\Uh{{\hat{\U}}}
\def\a{{\abf}}
\def\d{{\dbf}}
\def\s{{\sbf}}
\def\x{{\xbf}}
\def\y{{\ybf}}
\def\at{{\tilde{\abf}}}
\def\bt{{\tilde{\bbf}}}
\def\ah{{\hat{\abf}}}
\def\th{{\theta}}
\def\thh{{\hat{\theta}}}
\def\thi{{\theta_i}}
\def\thih{{\hat{\theta}_i}}
\def\thk{{\theta_k}}
\def\thik{{\hat{\theta}_k}}
\def\ai{{\a(\theta_i)}}
\def\ath{{\a(\theta)}}
\def\aths{{\a^*(\theta)}}
\def\athT{{\a^T(\theta)}}
\def\ais{{\a^*(\theta_i)}}
\def\ait{{\a^T(\theta_i)}}
\def\ak{{\a(\theta_k)}}
\def\aks{{\a^*(\theta_k)}}
\def\akt{{\a^T(\theta_k)}}
\def\thbf{{\thetabf}}
\def\sbft{{\tilde{\sbf}}}
\def\thbft{{\tilde{\thbf}}}
\def\thbfh{{\hat{\thbf}}}
\def\rhobfh{{\hat{\rhobf}}}
\def\thbfhh{{\hat{\hat{\thbf}}}}
\def\etat{{\tilde{\eta}}}
\def\etabft{{\tilde{\etabf}}}
\def\etabfth{{\hat{\tilde{\etabf}}}}
\def\etabfhh{{\hat{\hat{\etabf}}}}
\def\etabfh{{\hat{\etabf}}}
\def\alphabfh{{\hat{\alphabf}}}
\def\Vh{{\hat{V}}}
\def\Vt{{\tilde{V}}}
\def\therr{{\hat{\theta}-\theta}}
\def\therrbf{{\hat{\thetabf}-\thetabf_0}}
\def\therrbfwsf{{\hat{\thetabf}_\WSF-\thetabf_0}}
\def\etaerr{{\hat{\eta}-\eta}}
\def\etaerrbf{{\hat{\etabf}-\etabf_0}}
\def\etabfhat{{\hat{\etabf}}}
\def\ebh{{\etabfhat}}
\def\ebz{{\etabf_0}}
\def\Capo{{\C^{pq}_{a,1}}}
\def\Capt{{\C^{pq}_{a,2}}}
\def\Cesp{{\C_\ES}}
\def\therri{{\thih-\thi}}
\def\therrk{{\thik-\thk}}
\def\Cxik{{\Cbf_{\xi,1}^{ik}}}
\def\CxikT{{\Cbf_{\xi,2}^{ik}}}
\def\Cxpq{{\Cbf_{\xi,1}^{pq}}}
\def\CxpqT{{\Cbf_{\xi,2}^{pq}}}
\def\Cxii{{\Cbf_{\xi,1}^{ii}}}
\def\CxiiT{{\Cbf_{\xi,2}^{ii}}}
\def\Cxi{{\Cbf_{\xi,1}^{i}}}
\def\CxiT{{\Cbf_{\xi,2}^{i}}}
\def\Cx{{\Cbf_{\xi,1}}}
\def\CxT{{\Cbf_{\xi,2}}}
\def\Cmu{{\Cbf_{\MU}}}
\def\Cmuf{{\Cbf_{\MUF}}}
\def\Cmuik{{\Cbf_{\MU,ik}}}
\def\Cwmu{{\Cbf_{\WMU}}}
\def\Cwmuik{{\Cbf_{\WMU,ik}}}
\def\Lsl{{\Lambdabf_s}}
\def\Ls{{\Lambdabf_s}}
\def\Lh{{\hat{\Lambdabf}}}
%\def\Lsh{{\hat{\Lambdabf}_s}}
\def\Lshat{{\Lsh}}
\def\Lnh{{\hat{\Lambdabf}_n}}
\def\Lnhi{{\hat{\Lambdabf}_n^{-1}}}
\def\Lst{{\tilde{\Lambdabf}_s}}
\def\Lnt{{\tilde{\Lambdabf}_n}}
\def\Lt{{\tilde{\Lambdabf}}}
\def\Ltilde{{\Lt}}
\def\Lo{{\overline{\Lambdabf}}}
\def\Cx{{\Cbf_{\xi,1}}}
\def\CxT{{\Cbf_{\xi,2}}}
\def\pht{{\tilde{\phi}}}
\def\gt{{\tilde{g}}}
\def\xt{{\tilde{x}}}
\def\yt{{\tilde{y}}}
\def\xbft{{\tilde{\xbf}}}
\def\ybft{{\tilde{\ybf}}}
\def\gtogk{{{\gt_k}\over{g_k}}}
\def\atoak{{{\tilde{a}_k}\over{a_k}}}
\def\w{{\omega}}
\def\EEP{{\Ebar_W^*\Ebar_W \Pbf_{\bar{\Psibf}^*}^\perp}}
\def\EPp{{\Ebar_W \P_{\bar{\Psibf}^*}^\perp}}
\def\EP{{\Ebar_W \P_{\bar{\Psibf}^*}}}
\def\Eyha{{{\hat{\Ebf}}_y^\phstar}}
\def\LPbar{{\Psibar^*(\Psibar\Psibar^*)^{-1}}}
\def\PPbar{{\Psibar^*(\Psibar\Psibar^*)^{-1}\Psibar}}
\def\ppij{{{\partial}\over{\Psibf_{ij}}}}
\def\Pho{{{\hat{\Psibf}}_1}}
\def\Phw{{{\hat{\Psibf}}_2}}
\def\Phh{{{\hat{\Psibf}}_3}}
\def\pho{{{\hat{\psibf}}_1}}
\def\phw{{{\hat{\psibf}}_2}}
\def\phh{{{\hat{\psibf}}_3}}
\def\Pbh{{{\hat{\Psibar}}}}
\def\Pti{{{\tilde{\Psibf}}_i}}
\def\Pbi{{{\hat{\Psibf}}_i}}
\def\pto{{{\tilde{\psibf}}_1}}
\def\ptw{{{\tilde{\psibf}}_2}}
\def\pth{{{\tilde{\psibf}}_3}}
\def\Pto{{{\tilde{\Psibf}}_1}}
\def\Ptw{{{\tilde{\Psibf}}_2}}
\def\Pth{{{\tilde{\Psibf}}_3}}
\def\Pbt{{{\tilde{\Psibar}}}}
\def\En{{\Ebf_n}}
\def\Es{{\Ebf_s}}
\def\Ens{{\Ebf_n^*}}
\def\Ess{{\Ebf_s^*}}
\def\Eh{{\hat{\E}}}
\def\Et{{\tilde{\E}}}
\def\Ehh{{\hat{\hat{\E}}}}
\def\Ett{{\tilde{\tilde{\E}}}}
\def\Eshh{{\hat{\hat{\Ebf}}_s}}
\def\Enhh{{\hat{\hat{\Ebf}}_n}}
\def\Eshhs{{\hat{\hat{\Ebf}}_s^*}}
\def\Enhhs{{\hat{\hat{\Ebf}}_n^*}}
\def\Ent{{{\tilde{\Ebf}}_n}}
\def\Est{{{\tilde{\Ebf}}_s}}
\def\Entt{{\tilde{\tilde{\Ebf}}_n}}
\def\Estt{{\tilde{\tilde{\Ebf}}_s}}
\def\Entts{{\tilde{\tilde{\Ebf}}_n^*}}
\def\Estts{{\tilde{\tilde{\Ebf}}_s^*}}
\def\Ents{{{\tilde{\Ebf}}_n^*}}
\def\Ests{{{\tilde{\Ebf}}_s^*}}
\def\Enh{{\hat{\Ebf}_n}}
\def\Esh{{\hat{\Ebf}_s}}
\def\Enhs{{\hat{\Ebf}_n^*}}
\def\Eshs{{\hat{\Ebf}_s^*}}
\def\Eshz{{\hat{\Ebf}_0}}
\def\Esho{{\hat{\Ebf}_1}}
\def\Eshp{{\hat{\Ebf}_{p-1}}}
\def\EEs{{\Ebf_s^{}\Ebf_s^*}}
\def\EEsh{{\hat{\Ebf}_s^{}\hat{\Ebf}_s^*}}
\def\EEn{{\Ebf_n^{}\Ebf_n^*}}
\def\EEnh{{\hat{\Ebf}_n^{}\hat{\Ebf}_n^*}}
\newcommand{\ENEN}{\mbox{$\hat{\Ebf}_n^{}\hat{\Ebf}_n^*$}}
\def\EWE{{\Ebf_s^{}\Wbf\Ebf_s^*}}
\def\EWEh{{\hat{\Ebf}_s^{}\Wbf\hat{\Ebf}_s^*}}
\def\EWsEh{{\hat{\Ebf}_s^{}\Wbf_s^{}\hat{\Ebf}_s^*}}
\def\EWchEh{{\hat{\Ebf}_s^{}\hat{\Wbf}_c^{}\hat{\Ebf}_s^*}}
\def\EWot{{\Ebf_s \Wbf^{\half}}}
\def\EWoth{{\hat{\Ebf}_s^{} \Wbf^{\half}}}
\def\EWchoth{{\hat{\Ebf}_s^{} \hat{\Wbf}_c^{\half}}}
\def\et{{\tilde{\ebf}}}
\def\eh{{\hat{\ebf}}}
\def\ett{{\tilde{\tilde{\ebf}}}}
\def\ehh{{\hat{\hat{\ebf}}}}
\def\Wcot{{\Wbf_c^{\half}}}
\def\Wrot{{\Wbf_r^{\half}}}
\def\Deltaeq{{\stackrel{\Delta}{=}}}
\def\A{{\Abf}}
\def\B{{\Bbf}}
\def\C{{\Cbf}}
\def\D{{\Dbf}}
\def\E{{\Ebf}}
\def\F{{\Fbf}}
\def\G{{\Gbf}}
\def\H{{\Hbf}}
\def\I{{\Ibf}}
\def\It{{\tilde{\Ibf}}}
\def\J{{\Jbf}}
\def\K{{\Kbf}}
\def\L{{\Lbf}}
\def\M{{\Mbf}}
\def\N{{\Nbf}}
\def\P{{\Pbf}}
\def\Q{{\Qbf}}
\def\R{{\Rbf}}
\def\S{{\Sbf}}
\def\T{{\Tbf}}
\def\U{{\Ubf}}
\def\V{{\Vbf}}
\def\W{{\Wbf}}
\def\X{{\Xbf}}
\def\Y{{\Ybf}}
\def\Z{{\Zbf}}
\def\SNR{{\mbox{\rm SNR}}}
\def\ssSigma{{\scriptscriptstyle \Sigma}}
\def\CB{{\scriptscriptstyle CB}}
\def\CML{{\scriptscriptstyle CML}}
\def\UML{{\scriptscriptstyle UML}}
\def\DML{{\scriptscriptstyle DML}}
\def\SML{{\scriptscriptstyle SML}}
\def\ML{{\scriptscriptstyle ML}}
\def\MD{{\scriptscriptstyle MD}}
\def\MU{{\scriptscriptstyle MU}}
\def\MUF{{\scriptscriptstyle MUF}}
\def\MUD{{\scriptscriptstyle MUD}}
\def\MUDc{{\scriptscriptstyle MUDc}}
\def\WMU{{\scriptscriptstyle WMU}}
\def\MO{{\scriptscriptstyle MO}}
\def\ES{{\scriptscriptstyle ES}}
\def\MSE{{\scriptscriptstyle MSE}}
\def\LS{{\scriptscriptstyle LS}}
\def\TLS{{\scriptscriptstyle TLS}}
\def\BF{{\scriptscriptstyle BF}}
\def\FS{{\scriptscriptstyle FS}}
\def\AR{{\scriptscriptstyle AR}}
\def\WSF{{\scriptscriptstyle WSF}}
\def\OSF{{\scriptscriptstyle OSF}}
\def\SSF{{\scriptscriptstyle SSF}}
\def\RSF{{\scriptscriptstyle RSF}}
\def\NSF{{\scriptscriptstyle NSF}}
\def\MAP{{\scriptscriptstyle MAP}}
\def\OPT{{\scriptscriptstyle OPT}}
\def\FA{{\scriptscriptstyle FA}}
\def\SSE{{\scriptscriptstyle SSE}}
\def\LCMV{{\scriptscriptstyle LCMV}}
\def\SC{{\scriptscriptstyle SC}}
\def\WLS{{\scriptscriptstyle WLS}}
\def\aQa{{\abf^*\Qbf^{-1}\abf}}
\def\dQa{{\dbf^*\Qbf^{-1}\abf}}
\def\aQd{{\abf^*\Qbf^{-1}\dbf}}
\def\dQd{{\dbf^*\Qbf^{-1}\dbf}}
\def\zerobf{{\bf 0}}
\def\onebf{{\bf 1}}
\def\half{{\frac{1}{2}}}
\def\halfT{{{*}\over{2}}}
\def\jhalf{{{j}\over{2}}}
\def\mjhalf{{{-j}\over{2}}}
\def\mhalf{{-\half}}
\def\Rss{{\Rbf_{ss}}}
\def\Rssi{{\Rbf_{ss}^{-1}}}
\def\Rsst{{\R_{\sbf\tilde{s}}}}
\def\RsstH{{\R_{\sbf\tilde{s}}^*}}
\def\Rssb{{\Rbf_{\sbf\sbf}}}
\def\Rssbi{{\Rbf_{\sbf\sbf}^{-1}}}
\def\Rssd{{\Rbf_{\sbf s_d}}}
\def\RssdH{{\Rbf_{\sbf s_d}^*}}
\def\Rssh{{\hat{\Rbf}_{ss}}}
\def\Rxs{{\Rbf_{xs}}}
\def\Rxsb{{\Rbf_{\xbf\sbf}}}
\def\RxsH{{\Rbf_{x\sh}}}
\def\Rxx{{\Rbf_{xx}}}
\def\Rxxb{{\Rbf_{\xbf\xbf}}}
\def\Rxxbi{{\Rbf_{\xbf\xbf}^{-1}}}
\def\Rxxh{{\hat{\Rbf}_{xx}}}
\def\Ryyh{{\hat{\Rbf}_{yy}}}
\def\Rysh{{\hat{\Rbf}_{ys}}}
\def\Rxxo{{\Rbf_{xx0}}}
\def\Rzz{{\Rbf_{zz}}}
\def\Rzzh{{\hat{\Rbf}_{zz}}}
\def\Rh{{\hat{\R}}}
\def\Rhi{{\hat{\R}^{-1}}}
\def\Rhat{{\Rh}}
\def\Sh{{\hat{\S}}}
\def\St{{\tilde{\S}}}
\def\Xh{{\hat{\X}}}
\def\Xt{{\tilde{\X}}}
\def\Ad{{\A^\dag}}
\def\Adt{{\A^{\dag *}}}
\def\Sd{{\S^\dag}}
\def\Sdt{{\S^{\dag *}}}
\def\Th{{\hat{\T}}}
\def\Wh{{\hat{\W}}}
\def\Wt{{\tilde{\W}}}
\def\Rt{{\tilde{\R}}}
\def\Rhs{{\Rh^{}_\Sigma}}
%%\def\Rs{{\R^{}_\Sigma}}
\def\PAp{{\P_A^\perp}}
\def\PA0p{{\P_{A_0}^\perp}}
\def\PAs{{\P^{}_{{\Sigma^\mhalf A}}}}
\def\PAps{{\P^\perp_{{\Sigma^\mhalf A}}}}
\def\Pas{{\P^{}_{{\Sigma^\mhalf a(\theta)}}}}
\def\Paps{{\P^\perp_{{\Sigma^\mhalf a(\theta)}}}}
\def\DA{{\Delta\A}}
\def\Dt{{\Deltabf}}
\def\Sgbf{{\Sigmabf}}
\def\Sgbfh{{\hat{\Sigmabf}}}
\def\Sgbft{{\tilde{\Sgbf}}}
\def\Sgot{{\Sgbf^\mhalf}}
\def\Sgotm{{\Sgbf^\half}}
\def\Sgi{{\Sgbf^{-1}}}
\def\sg{{\sigma}}
\def\snt{{\sigma_n^2}}
\def\sdt{{\sigma_d^2}}
\def\snth{{\hat{\sigma}_n^2}}
\def\sat{{\sigma_a^2}}
\def\stwo{{\sigma^2}}
\def\s2h{{\hat{\sigma}^2}}
\def\Trss{{\Tr(\Rss)}}
\def\real{{\mbox{\rm real}}}
\def\imag{{\mbox{\rm imag}}}
\def\diag{{\mbox{\rm diag}}}
\def\spann{{\mbox{\rm span}}}
\def\Re{{\mbox{\rm Re}}}
\def\Im{{\mbox{\rm Im}}}
\def\Tr{{\mbox{\rm Tr}}}
\def\vecc{{\mbox{\rm vec}}}
\def\det{{\mbox{\rm det}}}
\def\rank{{\mbox{\rm rank}}}
\def\ba{\begin{array}}
\def\ea{\end{array}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\beas{\begin{eqnarray*}}
\def\eeas{\end{eqnarray*}}
\newcommand{\onempphp}[1]{
  \iftwocol  \unitlength .45pt
    \[\begin{picture}(440,320)(0,0)
     \special{psfile=#1 hscale=45 vscale=45 voffset=-10}%
    \end{picture}\]
  \else  \unitlength .8pt
    \begin{center} \begin{picture}(440,290)(0,0)
     \special{psfile=#1 hscale=.90 vscale=.80 hoffset=-20 voffset=-25}%
    \end{picture} \end{center}
  \fi
}

% Local Variables:
% mode: plain-tex
% TeX-master: t
% End:

